Collaborative Filtering and Multi-Label Classification with Matrix Factorization

Machine learning techniques for Recommendation System (RS) and Classification has become a prime focus of research to tackle the problem of information overload. RS are software tools that aim at making informed decisions about the services that a user may like. On the other hand, classification technique deals with the categorization of a data object into one of the several predefined classes. In the multi-label classification problem, unlike the traditional multi-class classification setting, each instance can be simultaneously associated with a subset of labels. The focus of thesis is on the development of novel techniques for collaborative filtering and multi-label classification. We propose a novel method of constructing a hierarchical bi-level maximum margin matrix factorization to handle matrix completion of ordinal rating matrix. Taking the cue from the alternative formulation of support vector machines, a novel loss function is derived by considering proximity as an alternative criterion instead of margin maximization criterion for matrix factorization framework. We extended the concept of matrix factorization for yet another important problem of machine learning namely multi-label classification which deals with the classification of data with multiple labels. We propose a novel piecewise-linear embedding method with a low-rank constraint on parametrization to capture nonlinear intrinsic relationships that exist in the original feature and label space. We also study the embedding of labels together with the group information with an objective to build an efficient multi-label classifier. We assume the existence of a low-dimensional space onto which the feature vectors and label vectors can be embedded. We ensure that labels belonging to the same group share the same sparsity pattern in their low-rank representations.

==> 0_frontmatter/dedication.tex <==
% Thesis Dedictation ---------------------------------------------------

\begin{dedication} %this creates the heading for the dedication page


\end{dedication}

% ---------------------------------------------------------------------- 


==> 0_frontmatter/glossary.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

% Glossary entries are defined with the command \nomenclature{1}{2}
% 1 = Entry name, e.g. abbreviation; 2 = Explanation
% You can place all explanations in this separate file or declare them in the middle of the text. Either way they will be collected in the glossary.

% required to print nomenclature name to page header
\markboth{\MakeUppercase{\nomname}}{\MakeUppercase{\nomname}}


% ----------------------- contents from here ------------------------

% chemicals
\nomenclature{ABC}{Artificial Bee Colony} 




==> 0_frontmatter/vineet-modified-abstract.tex <==
%\documentclass[PhD]{iitmdiss}
%\begin{document}
\begin{abstract}
Machine learning techniques for Recommendation System and Classification has become a prime focus of research to tackle the problem of information overload. Recommender Systems are software tools that aim at making informed decisions about the services that a user may like. Recommender Systems can be broadly classified into two categories namely, \emph{content-based filtering} and \emph{collaborative filtering}. In content-based filtering, users and items are represented using a set of features (profile) and an item is recommended by finding the similarity between the user and item profile. On the other hand in collaborative filtering, the user-item association is obtained based on the preferences of the user given so far and the preference information of other users. 

Classification technique deals with the categorization of a data object into one of the several predefined classes. The majority of the methods for supervised machine learning proceeds from a formal setting in which data objects (instances) are represented in the form of feature vectors wherein each object is associated with a unique class label from a set of disjoint class labels. Depending on the total number of disjoint classes, a learning task is categorized as binary classification or multi-class classification. In the multi-label classification problem, unlike the traditional multi-class classification setting,  each instance can be simultaneously associated with a subset of labels. 

In both recommendation and classification problem, the initial assumption is that the input-data is in the form of matrices which are inherently low rank. The key technical challenge involved in designing new algorithms for recommendation and classification is dependent on how well one can handle the huge and sparse matrices which usually has thousands to millions of rows and which are usually noisy. Recent years have witnessed extensive applications of low-rank linear factor model for exploiting the complex relationships that exist in such data matrices. The goal is to learn a low-dimensional embedding where the data object can be represented with a small number of features. Matrix factorization methods have attracted significant attention for learning the low-rank latent factors. The focus of thesis is on the development of novel techniques for collaborative filtering and multi-label classification.

In maximum margin matrix factorization scheme of collaborative filtering, ratings matrix with multiple discrete values is treated by specially extending hinge loss function to suit multiple levels. We view this process as analogous to extending two-class classifier to a unified multi-class classifier. Alternatively, multi-class classifier can be built by arranging multiple two- class classifiers in a hierarchical manner. We investigate this aspect for collaborative filtering and propose a novel method of constructing a hierarchical bi-level maximum margin matrix factorization to handle matrix completion of ordinal rating matrix. The advantages of the proposed method over other matrix factorization based collaborative filtering methods are given by detailed experimental analysis. We also observe that there could be several possible alternative criteria to formulate the factorization problem of discrete ordinal rating matrix, other than the maximum margin criterion. Taking the cue from the alternative formulation of support vector machines, a novel loss function is derived by considering \textit{proximity} as an alternative criterion for matrix factorization framework. We validate our hypothesis by conducting experiments on real and synthetic datasets. 

We extended the concept of matrix factorization for yet another important problem of machine learning namely multi-label classification which deals with the classification of data with multiple labels. We propose a novel piecewise-linear embedding method with a low-rank constraint on parametrization to capture nonlinear intrinsic relationships that exist in the original feature and label space. Extensive comparative studies to validate the effectiveness of the proposed method against the state-of-the-art multi-label learning approaches is given through detailed experimental analysis. We also study the embedding of labels together with the group information with an objective to build an efficient multi-label classifier. We assume the existence of a low-dimensional space onto which the feature  vectors and label vectors can be embedded. We ensure that labels belonging to the same group share the same sparsity pattern in their low-rank representations. We perform comparative analysis which manifests the superiority of our proposed method over state-of-art algorithms for multi-label learning. 
\end{abstract}
%\end{abstractlongs}
% ----------------------------------------------------------------------
%\end{document}

